Axial algebras of Monster type $(2\eta, \eta)$ for $D$ diagrams. I

Axial algebras are a class of commutative algebras generated by idempotents, with adjoint action semisimple and satisfying a prescribed fusion law. Axial algebras were introduced by Hall, Rehren, and Shpectorov in 2015 as a broad generalization of Majorana algebras of Ivanov, whose axioms were derived from the properties of the Griess algebra for the Monster group. The class of Matsuo algebras was introduced by Matsuo and later generalized by Hall, Rehren, and Shpectorov. A Matsuo algebra $M$ is built by a set of 3-transpositions $D$. Elements of $D$ are idempotents in $M$ and called axes. In particular, $M$ is an example of an axial algebra. It is known that double axes, i.e., sums of two orthogonal axes in a Matsuo algebra, satisfy the fusion law of Monster type. This observation shows that a set consisting of axes and double axes can generate a subalgebra of Monster type in the Matsuo algebra. Subalgebras corresponding to various series of 3-transposition groups are extensively studied by many authors. In this paper, we study primitive subalgebras generated by a single axis and two double axes. We classify all such subalgebras in seven out of nine possible cases for a diagram on 3-transpositions that are involved in the generating elements. We also construct several infinite series of axial algebras of Monster type generalizing our 3-generated algebras.

==> D6.tex <==
Suppose that the diagram on $Z$ is $D_6$. 
Clearly, $a$ is in the center of $\hat G$, and other elements form subdiagram  of type $B_6$ in terms of 2-generated subalgebras (see Subsection 5.4 in \cite{gjmss}). 
Therefore, $G=G(p) = \langle a \rangle \times \hat H / \langle (b^dc^e)^p=1 \rangle $, where $\hat{H}$ is the Coxeter group defined by the subdiagram with support $\{b,c,d,e \}$ and $p \in \{1,2,3\}$.

Note that $x$ cannot lie in the subalgebra $\dla y,z\dra$, since $a$ and $b$ are not conjugated in $G$. 
Therefore, $A$ decomposes as $\dla x\dra\oplus\dla y,z\dra$. Using classification of algebras for type $B_6$, we find that $A=\mathbb{F}\oplus A_p$, where $p\in\{1,2,3\}$ and $A_1$ is the 3-dimensional Matsuo algebra $3C(2\eta)$,
$A_2$ is the 5-dimensional algebra \cite[Table 7]{gjmss},
$A_3$ is the 8-dimensional algebra \cite[Table 8]{gjmss}.
